Breaks and Code Quality: Investigating the Impact of Forgetting on Software Development. A Registered Report

Developers interrupting their participation in a project might slowly forget critical information about the code, such as its intended purpose, structure, the impact of external dependencies, and the approach used for implementation. Forgetting the implementation details can have detrimental effects on software maintenance, comprehension, knowledge sharing, and developer productivity, resulting in bugs, and other issues that can negatively influence the software development process. Therefore, it is crucial to ensure that developers have a clear understanding of the codebase and can work efficiently and effectively even after long interruptions. This registered report proposes an empirical study aimed at investigating the impact of the developer's activity breaks duration and different code quality properties. In particular, we aim at understanding if the amount of activity in a project impact the code quality, and if developers with different activity profiles show different impacts on code quality. The results might be useful to understand if it is beneficial to promote the practice of developing multiple projects in parallel, or if it is more beneficial to reduce the number of projects each developer contributes.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> Section/Background.tex <==
\section{Background}
\label{sec:Background}

\todo[inline]{@Andrea}
Figure \ref{fig:ForgettingCurve} has a typical representation of a forgetting curve.

\begin{figure}[h]
    \centering
    \includegraphics[width=.9\columnwidth]{Figure/ebbinghaus1.pdf}
    \caption{Ebbinghaus curve with spaced repetition}
    \label{fig:ForgettingCurve}
\end{figure}


% The first experiments of the forgetting curve were performed by Ebbingaus [7]. Ebbinghaus and Bussenius [20] conducted an experiment that sought the relationship between forgetfulness and the passage of time. Nembhad and Osothsilp [21] studied the 14 main existing forgetting curve models. The authors divide the models into two groups. The first highlights the statistical models - which require parameter estimation using previously known forgetfulness cases to predict memory retention. And the second group has deterministic models - which do not depend on calculations of previous cases, being only a function of time. As an example, we cite the Learning- Forgetting Curve Models (LFCM). Averell and Heathcote [22] define a generic way of defining forgetting curves, such as:

% ADD FORMULA


% R(t) represents the retention of memory as a function of time t, a and b are parameters and P(t) represents a power function. also as a function of t. a, b, and P(t) are values between 0 and 1. Consequently, R(t) can also be interpreted as the probability of forgetting something that was learned after a time t. (t) classical, initially estimated by Ebbinghaus [7] is presented below, where are variable and adjustable parameters.


% ADD FORMULA


% The authors seek to define the values for these parameters according to experiments performed with volunteers. Based on the experiments, they estimate the values a = 0.19, b = 0.78, $\beta$ = 0.68, and hence the following forgetting curve:


% ADD FORMULA


% This curve represents the possibility of forgetting something that has already been learned. Thus, before the time t = 0. It is observed that the memory loss between the time t = 0 and t = 1 is much greater than between the following moments. This is because of the way the human brain works: information retention drops considerably in the first few moments of time and this rate decreases over time [7][23].



==> Section/Discussion.tex <==
\section{Discussion}
\label{sec:Discussion}

